$\nu$-Analysis: A New Notion of Robustness for Large Systems with Structured Uncertainties

We present a new, scalable alternative to the structured singular value, which we call $\nu$, provide a convex upper bound, study their properties and compare them to $\ell_1$ robust control. The analysis relies on a novel result on the relationship between robust control of dynamical systems and non-negative constant matrices.

==> figures/small-gain-thm.tex <==
\begin{tikzpicture}[node distance = 4em, line width=0.5mm, inner ysep=6pt, >=latex]
	\node [block, align = center] (sys) {$\mathbf H$};
	\node[block, above of = sys, align = center] (delta) {$\mathbf G$};
	\node[sum, left of = delta] (sum1) {$+$};
	\node[sum, right of = sys] (sum2) {$+$};
    \node[coordinate, left of = sum1] (in1) {};
    \node[coordinate, right of = sum2] (in2) {};
    
    % Feedback loop    
	\draw[->] (sys) -| node[pos=0.2, above] {$y_1$} (sum1);
	\draw[->] (sum1) -- node[above] {$e_1$} (delta);
	\draw[->] (delta) -| node[pos=0.2, above] {$y_2$} (sum2);
	\draw[->] (sum2) -- node[above] {$e_2$} (sys);
	
	% Inputs
	
	\draw[->] (in1) -- node[above] {$u_1$} (sum1);
	\draw[->] (in2) -- node[above] {$u_2$}(sum2);
\end{tikzpicture}

==> tex_files/A1_Notation.tex <==
\section*{Notation}
\begin{tabular}{cp{0.4\textwidth}}
  $\mathbf G$ & Linear time-invariant operator used in the definition and statements about $\nu$ and $\mu$ \\
  $M$ & Magnitude matrix. The element on the $i$th row and $j$th column $m_{ij} = \|\mathbf g_{ij}\|_1$ \\
  $\mathbf \Delta$ & Linear time-varying diagonal operator with diagonal elements $\delta_{ii}$ for $i = 1, \ldots, n$ \\
  $\Delta$ & Constant diagonal $n\times n$-dimensional matrix used for proofs in the static case (maybe).\\
  $\rho$ & Given a matrix $A \in \C^{n \times n}$, $\rho(A)$ denotes the spectral radius.
  
\end{tabular}\\

==> tex_files/A2_induced_norms.tex <==

We introduce a novel space for discrete-time vector-valued signals and show that for diagonal uncertainties, the induced norms on the plant and the uncertainties are \emph{separable}.
Finally we introduce and study a new $\mu$, called $\nu$, that allows us to characterize robustness for large-scale systems and structured uncertainty.


\subsection{Dynamical systems}
In this section we will introduce the $\kay_p$-space.
\begin{definition}[$\kay_p$]
    For a signal $x \in E^n$, we define the $\kay_p$-norm
    \[
        \|x\|_{\kay_p} = \begin{cases}
        \left(\sum_{i = 1}^n \left(\sup_t |x_i(t)|\right)^p \right)^{\frac{1}{p}}, & 1 \leq p < \infty \\
        \max_i\sup_t|x_i(t)|, & p = \infty.
        \end{cases}
    \]
\end{definition}
We think of the $\kay_p$-norm as taking the $\ell_\infty$ norm element wise, followed by the $\ell_p$-norm on the resulting finite-dimensional vector.
\begin{theorem}[Induced $\kay_p$ norms]
    Let $\mathbf G : \ell_{\infty, e}^n \to \ell_{\infty, e}^n$ be a linear time-varying causal operator and $M_G$ its magnitude matrix. Then,
    \begin{align}
        \|\mathbf G\|_{\kay_1 \to \kay_1} & = \max_j\sum_{i=1}^n M_{ij}, \\
        \|\mathbf G\|_{\kay_1 \to \kay_\infty} & = \max_{i, j}M_{ij}, \\
        \|\mathbf G\|_{\kay_\infty \to \kay_\infty} & = \max_i\sum_{j=1}^n M_{ij}.
    \end{align}
    
    If in addition, $\mathbf G$ is nonzero only on the diagonal, then
    \begin{equation}
         \|\mathbf G\|_{\kay_\infty \to \kay_1} = \sum_{i=1}^n M_{ii}.
    \end{equation}
\end{theorem}

\begin{proof}
\Blue{Write proof}
\end{proof}

As these are induced norms, the following submultiplicative identities are immediate.
\begin{prop}
    Let $\mathbf G, \mathbf H : \ell_{\infty, e}^n \to \ell_{\infty, e}^n$ be a linear time-varying causal operators. Then
    \begin{align}
        \|GH\|_{\kay_1 \to \kay_1} & \leq \|G\|_{\kay_1 \to \kay_1}\|H\|_{\kay_1 \to \kay_1} \\
        \|GH\|_{\kay_1 \to \kay_1} & \leq \|G\|_{\kay_\infty \to \kay_1}\|H\|_{\kay_1 \to \kay_\infty} \\
        \|GH\|_{\kay_\infty \to \kay_\infty} & \leq \|G\|_{\kay_\infty \to \kay_\infty}\|H\|_{\kay_\infty \to \kay_\infty} \\
        \|GH\|_{\kay_\infty \to \kay_\infty} & \leq \|G\|_{\kay_1 \to \kay_\infty}\|H\|_{\kay_\infty \to \kay_1}
    \end{align}
\end{prop}

Since $\kay_p$ norms reduce to $\ell_p$ norms on finite-dimensional vectors, they are all equivalent. The ones we care about obey
\begin{prop}
\label{prop:equivalence_vector_norms}
    For $x \in \ell_{\infty}^n$
    \begin{equation}
        \|x\|_{\kay_\infty} \leq \|x\|_{\kay_1} \leq n \|x\|_{\kay_\infty}
    \end{equation}
\end{prop}

This means that the induced norms are equivalent as well:
\begin{prop}
\label{prop:equivalence_operator_norms}
    Let $G : \ell_{\infty}^n \to \ell_\infty^n$ then
    \begin{align*}
        \|\mathbf G\|_{\kay_1 \to \kay_\infty} & \leq
        \|\mathbf G\|_{\kay_\infty \to \kay_\infty} \leq
        \|\mathbf G\|_{\kay_\infty \to \kay_1} \\
        \frac{1}{n}\|\mathbf G\|_{\kay_\infty \to \kay_1} & \leq
        \|\mathbf G\|_{\kay_1 \to \kay_1}\leq
        n\|\mathbf G\|_{1 \to \kay_\infty} \\
        \frac{1}{n}\|\mathbf G\|_{\kay_\infty \to \kay_1} & \leq \|\mathbf G\|_{\kay_\infty \to \kay_\infty}
    \end{align*}
\end{prop}
We now have the necessary machinery to study structured uncertainties.
